Polynomial chaos expansions for dependent random variables

Polynomial chaos expansions (PCE) are well-suited to quantifying uncertainty in models parameterized by independent random variables. The assumption of independence leads to simple strategies for evaluating PCE coefficients. In contrast, the application of PCE to models of dependent variables is much more challenging. Three approaches can be used. The first approach uses mapping methods where measure transformations, such as the Nataf and Rosenblatt transformation, can be used to map dependent random variables to independent ones; however we show that this can significantly degrade performance since the Jacobian of the map must be approximated. A second strategy is the class of dominating support methods which build PCE using independent random variables whose distributional support dominates the support of the true dependent joint density; we provide evidence that this approach appears to produce approximations with suboptimal accuracy. A third approach, the novel method proposed here, uses Gram-Schmidt orthogonalization (GSO) to numerically compute orthonormal polynomials for the dependent random variables. This approach has been used successfully when solving differential equations using the intrusive stochastic Galerkin method, and in this paper we use GSO to build PCE using a non-intrusive stochastic collocation method. The stochastic collocation method treats the model as a black box and builds approximations of model output from a set of samples. Building PCE from samples can introduce ill-conditioning which does not plague stochastic Galerkin methods. To mitigate this ill-conditioning we generate weighted Leja sequences, which are nested sample sets, to build accurate polynomial interpolants. We show that our proposed approach produces PCE which are orders of magnitude more accurate than PCE constructed using mapping or dominating support methods.

==> defs.tex <==
\def\rv{Z}  %random variable
\def\rvd{z}  %random variable dummy variable
\def\brv{Z} %random vector
\def\pbwt{\omega} % probability measure
\newcommand{\norm}[2]{\left\lVert #1 \right\rVert_{#2}}
\newcommand{\V}[1]{{\boldsymbol{#1}}}
\def\samples{Z_M}
\def\R{\mathbb{R}}
\def\N{\mathbb{N}}
\def\nodes{\mathcal{Z}}
\newcommand{\brvsamp}[1]{\brv^{(#1)}}
\newcommand{\rvdsamp}[1]{\rvd^{(#1)}}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\dx}[1]{\mathrm{d}#1}
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}

\def\urv{U}
\def\burv{U}
\def\urvd{u}

\def\Rvx{R^{\brv}}
\def\Rvy{{R^{V}}}

\def\dom{\Omega}
\def\rotation{A}



